MaMaDroid2.0 -- The Holes of Control Flow Graphs

Android malware is a continuously expanding threat to billions of mobile users around the globe. Detection systems are updated constantly to address these threats. However, a backlash takes the form of evasion attacks, in which an adversary changes malicious samples such that those samples will be misclassified as benign. This paper fully inspects a well-known Android malware detection system, MaMaDroid, which analyzes the control flow graph of the application. Changes to the portion of benign samples in the train set and models are considered to see their effect on the classifier. The changes in the ratio between benign and malicious samples have a clear effect on each one of the models, resulting in a decrease of more than 40% in their detection rate. Moreover, adopted ML models are implemented as well, including 5-NN, Decision Tree, and Adaboost. Exploration of the six models reveals a typical behavior in different cases, of tree-based models and distance-based models. Moreover, three novel attacks that manipulate the CFG and their detection rates are described for each one of the targeted models. The attacks decrease the detection rate of most of the models to 0%, with regards to different ratios of benign to malicious apps. As a result, a new version of MaMaDroid is engineered. This model fuses the CFG of the app and static analysis of features of the app. This improved model is proved to be robust against evasion attacks targeting both CFG-based models and static analysis models, achieving a detection rate of more than 90% against each one of the attacks.

==> drr_black_1nn.tex <==
x y
0.1 0.5873015873015889
0.2 0.4914529914529879
0.3 0.4694749694749636
0.4 0.42857142857142366
0.5 0.41391941391940856
0.6 0.40293040293039795
0.7 0.38278388278387804
0.8 0.39010989010988495
0.9 0.39133089133088617
1.0 0.37667887667887284

==> drr_black_3nn.tex <==
x y
0.1 0.5505189255189299
0.2 0.44398656898656763
0.3 0.41417378917378855
0.4 0.38949938949938856
0.5 0.3784086284086269
0.6 0.3721509971509954
0.7 0.3650793650793634
0.8 0.3621794871794852
0.9 0.36034798534798296
1.0 0.3559218559218544

==> drr_black_5nn.tex <==
x y
0.1 0.5314102564102504
0.2 0.42793040293039564
0.3 0.39850427350426726
0.4 0.38137973137972575
0.5 0.3707264957264905
0.6 0.3653235653235603
0.7 0.35921855921855467
0.8 0.3567155067155023
0.9 0.35558608058607616
1.0 0.35323565323564904

==> drr_black_ada.tex <==
x y 
0.1 0.5255688034188037
0.2 0.5140366758241774
0.3 0.5103349358974372
0.4 0.503642261904761
0.5 0.5033012667887643
0.6 0.5025579212454216
0.7 0.4946569902319927
0.8 0.5017784493284507
0.9 0.5013989621489634
1.0 0.5008973595848607

==> drr_black_dt.tex <==
x y 
0.1 0.48412698412697835
0.2 0.4047619047619001
0.3 0.36202686202685785
0.4 0.3620268620268586
0.5 0.3748473748473708
0.6 0.3864468864468813
0.7 0.372405372405368
0.8 0.3687423687423649
0.9 0.3986568986568929
1.0 0.373626373626369

==> drr_black_rf.tex <==
x y 
0.1 0.444164599389346
0.2 0.40009544869711966
0.3 0.38695958411588643
0.4 0.3730923649484033
0.5 0.3696440745452308
0.6 0.3658472754118344
0.7 0.36100869319195344
0.8 0.3626980477728456
0.9 0.35790086386840203
1.0 0.35623976097431703

==> drr_clean_1nn.tex <==
x y
0.1 0.6056166056166077
0.2 0.5024420024419992
0.3 0.4536019536019476
0.4 0.4218559218559164
0.5 0.4194139194139142
0.6 0.39316239316238843
0.7 0.3894993894993847
0.8 0.38644688644688174
0.9 0.38217338217337743
1.0 0.3785103785103739

==> drr_clean_3nn.tex <==
x y
0.1 0.5543854293854333
0.2 0.45838420838420757
0.3 0.4074582824582817
0.4 0.39514652014651874
0.5 0.3785612535612524
0.6 0.3700142450142431
0.7 0.36319698819698637
0.8 0.3634004884004863
0.9 0.3617724867724844
1.0 0.35464997964997724

==> drr_clean_5nn.tex <==
x y
0.1 0.5309218559218496
0.2 0.43681318681317916
0.3 0.39981684981684323
0.4 0.38461538461537864
0.5 0.37194749694749146
0.6 0.36440781440780945
0.7 0.3601343101343056
0.8 0.35860805860805406
0.9 0.35476190476190045
1.0 0.3518925518925477

==> drr_clean_ada.tex <==
x y 
0.1 0.6745713522588533
0.2 0.6450560286935297
0.3 0.6123608669108669
0.4 0.587047435897436
0.5 0.5772789224664221
0.6 0.5716380799755795
0.7 0.5620572344322339
0.8 0.5386399420024419
0.9 0.5428565934065931
1.0 0.5332108821733823

==> drr_clean_dt.tex <==
x y 
0.1 0.9291819291819307
0.2 0.9133089133089152
0.3 0.9133089133089153
0.4 0.9078144078144098
0.5 0.8998778998779023
0.6 0.8992673992674011
0.7 0.9029304029304048
0.8 0.8980463980464002
0.9 0.8974358974358995
1.0 0.8949938949938973

==> drr_clean_rf.tex <==
x y 
0.1 0.7353249726419581
0.2 0.6359144433385303
0.3 0.5826749139424846
0.4 0.5365968997814371
0.5 0.5224757189202314
0.6 0.5159468186276501
0.7 0.4952805492738141
0.8 0.49135878798180566
0.9 0.4757260765523897
1.0 0.4777917743748721

==> drr_full_1nn.tex <==
x y
0.1 0.5964590964590982
0.2 0.5067155067155041
0.3 0.4529914529914468
0.4 0.4194139194139137
0.5 0.4188034188034136
0.6 0.4065934065934017
0.7 0.3956043956043907
0.8 0.37973137973137466
0.9 0.3736263736263692
1.0 0.3736263736263693

==> drr_full_3nn.tex <==
x y
0.1 0.5524013024013068
0.2 0.44810744810744735
0.3 0.4100529100529095
0.4 0.3884818884818869
0.5 0.3765771265771252
0.6 0.3760683760683743
0.7 0.36619861619861427
0.8 0.3563797313797294
0.9 0.3564306064306045
1.0 0.3553622303622281

==> drr_full_5nn.tex <==
x y
0.1 0.5438644688644625
0.2 0.4319902319902246
0.3 0.39942002442001784
0.4 0.38284493284492693
0.5 0.3697191697191644
0.6 0.36593406593406097
0.7 0.36361416361415905
0.8 0.35579975579975137
0.9 0.3546398046398003
1.0 0.3534798534798492

==> drr_full_ada.tex <==
x y 
0.1 0.5617666056166047
0.2 0.5327975274725277
0.3 0.5255099206349207
0.4 0.5154608363858373
0.5 0.5108620879120868
0.6 0.5082440170940165
0.7 0.5007089743589774
0.8 0.5039878357753366
0.9 0.5049515873015873
1.0 0.5029807387057383

==> drr_full_dt.tex <==
x y 
0.1 0.49023199023198566
0.2 0.4017094017093972
0.3 0.366300366300362
0.4 0.37301587301586886
0.5 0.3797313797313756
0.6 0.3894993894993848
0.7 0.39621489621489175
0.8 0.3766788766788723
0.9 0.41025641025640486
1.0 0.3797313797313756

==> drr_full_rf.tex <==
x y 
0.1 0.46139583713131965
0.2 0.40944061823498507
0.3 0.39649656446555803
0.4 0.38026717405535426
0.5 0.37511379618595486
0.6 0.3714853670466712
0.7 0.3650826800066038
0.8 0.367292086387933
0.9 0.3626332882786192
1.0 0.35971368020813016

==> drr_random_1nn.tex <==
x y
0.1 0.5952380952380977
0.2 0.48229548229547736
0.3 0.4450549450549391
0.4 0.43467643467642886
0.5 0.4114774114774058
0.6 0.3901098901098851
0.7 0.38583638583638113
0.8 0.39316239316238843
0.9 0.37728937728937284
1.0 0.3693528693528649

==> drr_random_3nn.tex <==
x y
0.1 0.5456349206349245
0.2 0.43859381359381316
0.3 0.40750915750915634
0.4 0.39514652014651913
0.5 0.378561253561252
0.6 0.3642653642653623
0.7 0.3619759869759848
0.8 0.36182336182336006
0.9 0.356837606837605
1.0 0.35648148148147935

==> drr_random_5nn.tex <==
x y
0.1 0.5267399267399209
0.2 0.4282356532356462
0.3 0.3971001221001157
0.4 0.3820818070818013
0.5 0.372313797313792
0.6 0.3619047619047573
0.7 0.35793650793650356
0.8 0.35805860805860346
0.9 0.3557997557997514
1.0 0.35262515262514843

==> drr_random_ada.tex <==
x y 
0.1 0.5855611416361437
0.2 0.5560724511599534
0.3 0.5395874542124549
0.4 0.531242582417582
0.5 0.5284211080586081
0.6 0.5232939255189243
0.7 0.5187983821733835
0.8 0.5107913614163619
0.9 0.5135511752136747
1.0 0.5103651862026873

==> drr_random_dt.tex <==
x y 
0.1 0.62759462759463
0.2 0.5854700854700856
0.3 0.5647130647130651
0.4 0.546398046398046
0.5 0.5384615384615373
0.6 0.5305250305250285
0.7 0.5256410256410243
0.8 0.5213675213675194
0.9 0.5170940170940147
1.0 0.5225885225885203

==> drr_random_rf.tex <==
x y 
0.1 0.5368967850109958
0.2 0.47046716328354227
0.3 0.44128401239679144
0.4 0.4188651915689079
0.5 0.4100794885056631
0.6 0.40535936925983185
0.7 0.3969304794165247
0.8 0.3951648403844403
0.9 0.38557063827094484
1.0 0.386697680746023

==> er_black_1nn.tex <==
x y
0.1 0.3772893772893773
0.2 0.2564102564102564
0.3 0.2032967032967033
0.4 0.13644688644688643
0.5 0.11996336996336997
0.6 0.09981684981684982
0.7 0.08424908424908426
0.8 0.06868131868131869
0.9 0.07326007326007326
1.0 0.06318681318681318

==> er_black_3nn.tex <==
x y
0.1 0.30036630036630035
0.2 0.13644688644688643
0.3 0.08058608058608059
0.4 0.045787545787545784
0.5 0.029304029304029304
0.6 0.027472527472527472
0.7 0.016483516483516484
0.8 0.013736263736263736
0.9 0.015567765567765568
1.0 0.009157509157509158

==> er_black_5nn.tex <==
x y
0.1 0.25274725274725274
0.2 0.07967032967032966
0.3 0.03205128205128205
0.4 0.0173992673992674
0.5 0.00641025641025641
0.6 0.007326007326007326
0.7 0.0009157509157509158
0.8 0.0009157509157509158
0.9 0.0009157509157509158
1.0 0.0

==> er_black_ada.tex <==
x y 
0.1 0.11813186813186813
0.2 0.056776556776556776
0.3 0.046703296703296704
0.4 0.029304029304029304
0.5 0.03021978021978022
0.6 0.03021978021978022
0.7 0.026556776556776556
0.8 0.028388278388278388
0.9 0.028388278388278388
1.0 0.0

==> er_black_dt.tex <==
x y 
0.1 0.32967032967032966
0.2 0.1446886446886447
0.3 0.05128205128205128
0.4 0.037545787545787544
0.5 0.056776556776556776
0.6 0.08516483516483517
0.7 0.07417582417582418
0.8 0.0641025641025641
0.9 0.0347985347985348
1.0 0.055860805860805864

==> er_black_rf.tex <==
x y 
0.1 0.05402930402930403
0.2 0.0
0.3 0.0
0.4 0.0
0.5 0.0
0.6 0.0
0.7 0.0
0.8 0.0
0.9 0.0
1.0 0.0

==> er_clean_1nn.tex <==
x y
0.1 0.38644688644688646
0.2 0.27014652014652013
0.3 0.16941391941391942
0.4 0.14743589743589744
0.5 0.11538461538461539
0.6 0.09340659340659341
0.7 0.08974358974358974
0.8 0.076007326007326
0.9 0.07326007326007326
1.0 0.06318681318681318

==> er_clean_3nn.tex <==
x y
0.1 0.3342490842490842
0.2 0.1401098901098901
0.3 0.07967032967032966
0.4 0.05036630036630037
0.5 0.03571428571428571
0.6 0.027472527472527472
0.7 0.009157509157509158
0.8 0.015567765567765568
0.9 0.014652014652014652
1.0 0.01098901098901099

==> er_clean_5nn.tex <==
x y
0.1 0.2793040293040293
0.2 0.09523809523809523
0.3 0.029304029304029304
0.4 0.0173992673992674
0.5 0.013736263736263736
0.6 0.00641025641025641
0.7 0.0018315018315018315
0.8 0.004578754578754579
0.9 0.0
1.0 0.0009157509157509158

==> er_clean_ada.tex <==
x y 
0.1 0.6996336996336996
0.2 0.5879120879120879
0.3 0.4606227106227106
0.4 0.3342490842490842
0.5 0.304029304029304
0.6 0.29304029304029305
0.7 0.24267399267399267
0.8 0.2032967032967033
0.9 0.16025641025641027
1.0 0.14743589743589744

==> er_clean_dt.tex <==
x y 
0.1 0.8965201465201466
0.2 0.8891941391941391
0.3 0.8690476190476191
0.4 0.8571428571428571
0.5 0.8543956043956044
0.6 0.8443223443223443
0.7 0.8424908424908425
0.8 0.8516483516483516
0.9 0.8415750915750916
1.0 0.836996336996337

==> er_clean_rf.tex <==
x y 
0.1 0.6904761904761905
0.2 0.47710622710622713
0.3 0.3360805860805861
0.4 0.2875457875457875
0.5 0.24267399267399267
0.6 0.2454212454212454
0.7 0.19597069597069597
0.8 0.18681318681318682
0.9 0.1749084249084249
1.0 0.16575091575091574

==> er_full_1nn.tex <==
x y
0.1 0.40384615384615385
0.2 0.2692307692307692
0.3 0.18956043956043955
0.4 0.1346153846153846
0.5 0.1282051282051282
0.6 0.10897435897435898
0.7 0.09432234432234432
0.8 0.07417582417582418
0.9 0.0641025641025641
1.0 0.0695970695970696

==> er_full_3nn.tex <==
x y
0.1 0.32875457875457875
0.2 0.13736263736263737
0.3 0.06776556776556776
0.4 0.047619047619047616
0.5 0.02564102564102564
0.6 0.03296703296703297
0.7 0.020146520146520148
0.8 0.009157509157509158
0.9 0.010073260073260074
1.0 0.009157509157509158

==> er_full_5nn.tex <==
x y
0.1 0.27197802197802196
0.2 0.08791208791208792
0.3 0.039377289377289376
0.4 0.02197802197802198
0.5 0.005494505494505495
0.6 0.004578754578754579
0.7 0.008241758241758242
0.8 0.0018315018315018315
0.9 0.0
1.0 0.0027472527472527475

==> er_full_ada.tex <==
x y 
0.1 0.2857142857142857
0.2 0.14835164835164835
0.3 0.12087912087912088
0.4 0.07783882783882784
0.5 0.04945054945054945
0.6 0.05311355311355311
0.7 0.054945054945054944
0.8 0.040293040293040296
0.9 0.03388278388278388
1.0 0.01098901098901099

==> er_full_dt.tex <==
x y 
0.1 0.3553113553113553
0.2 0.19230769230769232
0.3 0.08058608058608059
0.4 0.04304029304029304
0.5 0.045787545787545784
0.6 0.08424908424908426
0.7 0.10897435897435898
0.8 0.08241758241758242
0.9 0.06227106227106227
1.0 0.08058608058608059

==> er_full_rf.tex <==
x y 
0.1 0.05860805860805861
0.2 0.0
0.3 0.0
0.4 0.0
0.5 0.0
0.6 0.0
0.7 0.0
0.8 0.0
0.9 0.0
1.0 0.0

==> er_random_1nn.tex <==
x y
0.1 0.3782051282051282
0.2 0.23351648351648352
0.3 0.1575091575091575
0.4 0.14743589743589744
0.5 0.1108058608058608
0.6 0.07967032967032966
0.7 0.07509157509157509
0.8 0.0815018315018315
0.9 0.06318681318681318
1.0 0.056776556776556776

==> er_random_3nn.tex <==
x y
0.1 0.3131868131868132
0.2 0.11721611721611722
0.3 0.07142857142857142
0.4 0.057692307692307696
0.5 0.03296703296703297
0.6 0.016483516483516484
0.7 0.018315018315018316
0.8 0.016483516483516484
0.9 0.008241758241758242
1.0 0.013736263736263736

==> er_random_5nn.tex <==
x y
0.1 0.2445054945054945
0.2 0.08058608058608059
0.3 0.03571428571428571
0.4 0.016483516483516484
0.5 0.010073260073260074
0.6 0.00641025641025641
0.7 0.0018315018315018315
0.8 0.0018315018315018315
0.9 0.0027472527472527475
1.0 0.0018315018315018315

==> er_random_ada.tex <==
x y 
0.1 0.34706959706959706
0.2 0.23901098901098902
0.3 0.17307692307692307
0.4 0.1336996336996337
0.5 0.10531135531135531
0.6 0.10073260073260074
0.7 0.07967032967032966
0.8 0.08516483516483517
0.9 0.07051282051282051
1.0 0.05128205128205128

==> er_random_dt.tex <==
x y 
0.1 0.4413919413919414
0.2 0.3836996336996337
0.3 0.3360805860805861
0.4 0.3305860805860806
0.5 0.32234432234432236
0.6 0.3058608058608059
0.7 0.3067765567765568
0.8 0.2893772893772894
0.9 0.29120879120879123
1.0 0.28846153846153844

==> er_random_rf.tex <==
x y 
0.1 0.2967032967032967
0.2 0.17124542124542125
0.3 0.10531135531135531
0.4 0.07051282051282051
0.5 0.06776556776556776
0.6 0.06043956043956044
0.7 0.05860805860805861
0.8 0.05036630036630037
0.9 0.046703296703296704
1.0 0.04304029304029304

==> mr_black_1nn.tex <==
x y
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_black_3nn.tex <==
x y
0.1 0.5669138946492276
0.2 0.6875718001776392
0.3 0.7097215606128066
0.4 0.7814168378108484
0.5 0.8093954825710596
0.6 0.8420372347913063
0.7 0.8583581109014297
0.8 0.8647698836589781
0.9 0.8840052019316235
1.0 0.8904169746891719

==> mr_black_5nn.tex <==
x y
0.1 0.4618174392950972
0.2 0.5988778510892176
0.3 0.6537295345725707
0.4 0.7308611486447734
0.5 0.765026518838752
0.6 0.800865292535848
0.7 0.827855320826514
0.8 0.8392490966380836
0.9 0.8493145069045351
1.0 0.8600760144250018

==> mr_black_ada.tex <==
x y 
0.1 0.3069469037889563
0.2 0.30703532736935435
0.3 0.30711279442606376
0.4 0.30713400541563673
0.5 0.3071854726186076
0.6 0.30739857303482443
0.7 0.3074356161907488
0.8 0.30736480803774135
0.9 0.30733948852531834
1.0 0.3073659281356702

==> mr_black_dt.tex <==
x y 
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_black_rf.tex <==
x y 
0.1 0.41971735289377066
0.2 0.4872782763192912
0.3 0.5761204322933973
0.4 0.6522008547757501
0.5 0.6940902672250232
0.6 0.7021125602216576
0.7 0.7490978465650768
0.8 0.7503575600691348
0.9 0.7807028134428021
1.0 0.7882289273926331

==> mr_clean_1nn.tex <==
x y
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_clean_3nn.tex <==
x y
0.1 0.543015468916547
0.2 0.649684052064853
0.3 0.7213793292628947
0.4 0.7796681725133351
0.5 0.8058981519760333
0.6 0.8449516769538283
0.7 0.8571923340364208
0.8 0.8694329911190133
0.9 0.8752618754440573
1.0 0.9055720739342864

==> mr_clean_5nn.tex <==
x y
0.1 0.4605035256562019
0.2 0.581036745109806
0.3 0.6724073423035403
0.4 0.7236873120759643
0.5 0.7618188109955585
0.6 0.8100461293285576
0.7 0.8192125142150438
0.8 0.8362936939775292
0.9 0.8502309948597333
1.0 0.8686884118895206

==> mr_clean_ada.tex <==
x y 
0.1 0.30700967562221193
0.2 0.3069677311788297
0.3 0.30697825655655553
0.4 0.3069856114791585
0.5 0.30699878439353645
0.6 0.30701678129516163
0.7 0.3070394309730171
0.8 0.3070463482909941
0.9 0.3070678832396513
1.0 0.30708262570031764

==> mr_clean_dt.tex <==
x y 
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_clean_rf.tex <==
x y 
0.1 0.42611677550354987
0.2 0.42458688864773975
0.3 0.4358007133001429
0.4 0.4660634392159947
0.5 0.48903910725021194
0.6 0.496614130479615
0.7 0.49747474673991887
0.8 0.5083289302826695
0.9 0.5363018641053559
1.0 0.5385455402429611

==> mr_full_1nn.tex <==
x y
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_full_3nn.tex <==
x y
0.1 0.5535074607016263
0.2 0.6764969199600556
0.3 0.7213793292628947
0.4 0.7971548254884672
0.5 0.8140585900310949
0.6 0.8274650239786963
0.7 0.8612725530639517
0.8 0.886336755661641
0.9 0.8886683093916586
1.0 0.8962458590142159

==> mr_full_5nn.tex <==
x y
0.1 0.46567337267012165
0.2 0.596760655514726
0.3 0.6691836772196189
0.4 0.7274634592473482
0.5 0.7693087817099192
0.6 0.7931853402672554
0.7 0.813902062703582
0.8 0.8465490857982126
0.9 0.8508792203915642
1.0 0.8655589849154626

==> mr_full_ada.tex <==
x y 
0.1 0.30694422854928904
0.2 0.30699150398747554
0.3 0.3070629968210977
0.4 0.30707441900443
0.5 0.30714054488225473
0.6 0.307281072888251
0.7 0.3073300038460316
0.8 0.3072751217612728
0.9 0.30724732299886903
1.0 0.30726188366106433

==> mr_full_dt.tex <==
x y 
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_full_rf.tex <==
x y 
0.1 0.3812485390056063
0.2 0.44942652891796064
0.3 0.5280470274016758
0.4 0.6130200823888231
0.5 0.6607618318600035
0.6 0.6623580014056917
0.7 0.7169908511561625
0.8 0.7186152313066982
0.9 0.7492113143707408
1.0 0.7579750682735032

==> mr_random_1nn.tex <==
x y
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_random_3nn.tex <==
x y
0.1 0.545929911079069
0.2 0.6782455852575687
0.3 0.7476093087255928
0.4 0.7668446269982382
0.5 0.8187216974911302
0.6 0.8601067761989428
0.7 0.877593429174075
0.8 0.8729303217140397
0.9 0.8857538672291366
1.0 0.8985774127442335

==> mr_random_5nn.tex <==
x y
0.1 0.4548320789460144
0.2 0.5998262535258717
0.3 0.673687836126474
0.4 0.7206057568240904
0.5 0.7689607330829118
0.6 0.8188485083473083
0.7 0.8374944015968228
0.8 0.8311109003918917
0.9 0.8525381719884567
1.0 0.8704256443555487

==> mr_random_ada.tex <==
x y 
0.1 0.30701379007363294
0.2 0.30707227132274817
0.3 0.30713034194207034
0.4 0.30717167268844436
0.5 0.3071978007833338
0.6 0.3072888661108639
0.7 0.30728633557310026
0.8 0.30734199641282334
0.9 0.30736465592280504
1.0 0.30740627018686184

==> mr_random_dt.tex <==
x y 
0.1 1.0
0.2 1.0
0.3 1.0
0.4 1.0
0.5 1.0
0.6 1.0
0.7 1.0
0.8 1.0
0.9 1.0
1.0 1.0

==> mr_random_rf.tex <==
x y 
0.1 0.43387920006770875
0.2 0.5045238330001077
0.3 0.5490492437072378
0.4 0.5889741917701365
0.5 0.6223117117229559
0.6 0.6525453327356698
0.7 0.6602148044903152
0.8 0.6752089079065552
0.9 0.7014483999163781
1.0 0.7113429420689352
